Generation of complete test sets

We use testing to check if a combinational circuit N always evaluates to 0. The usual point of view is that to prove that N always evaluates to 0 one has to check the value of N for all 2^|X| input assignments where X is the set of input variables of N. We use the notion of a Stable Set of Assignments (SSA) to show that one can build a complete test set (i.e. a test set proving that N always evaluates to 0) that consists of less than 2^|X| tests. Given an unsatisfiable CNF formula H(W), an SSA of H is a set of assignments to W proving unsatisfiability of H. A trivial SSA is the set of all 2^|W| assignments to W. Importantly, real-life formulas can have SSAs that are much smaller than 2^|W|. Generating a complete test set for N using only the machinery of SSAs is inefficient. We describe a much faster algorithm that combines computation of SSAs with resolution derivation and produces a complete test set for a "projection" of N on a subset of variables of N. We give experimental results and describe potential applications of this algorithm.

==> junk.tex <==

\vspace{20pt}

just something to fill out the page
\clearpage
just something to fill out the page
\clearpage


==> qe.tbl.tex <==
%
%
\begin{wraptable}{l}{2.1in}
\small
\caption{\ti{Using \sas for quantifier elimination}}
\scriptsize
\begin{center}
%\begin{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|c|c|c|c|c|c|} \hline
name   & \#vars           & \#free\_   &result      & other & \sas     \\ 
        &                  & vars      & (\#cls)    &  (s.)    &  (s.)    \\ \hline

        &              &             &      &          &           \\ \hline
   
 
\end{tabular}                
\end{center}
\label{tbl:ec_by_lor}
\vspace{-5pt}
%\end{table}
\end{wraptable}


==> s0torage.tex <==
Assume that $F$ is a CNF formula. (We will use this assumption for all
the formulas considered in this paper.) An example of the structural
property is the redundancy of a clause $C$ in $F$. Indeed, suppose that
formulas $F$ and $G$ contain clause $C$ and $F \equiv G$. The fact
that $C$ is implied by $F \setminus \s{C}$ does not mean that $C$ is
implied $G \setminus \s{C}$. An example of a semantic property is an
implication. If $C$ is implied by $F$ and $F \equiv G$, then $C$ is
implied by $G$ as well.

--------------------

An example of a semantic property is implication. If $C$ is implied by
$F$ and $F \equiv G$, then $C$ is implied by $G$ as well. An
interpolant is an example of a structural property.  Suppose that
$J(Y)$ is an interpolant for formula $A(X,Y) \wedge B(Y,Z)$ i.e.  $A
\rightarrow I$ and $I \rightarrow \overline{B}$.  Formula $J$ may not
be an interpolant for $A'(X,Y) \wedge B'(Y,Z)$ logically equivalent to
$A \wedge B$ if, for instance, $A \not\equiv A'$ and/or $B \not\equiv
B'$.

-----
Let us consider the challenges of purely semantic derivation by the
example of propositional SAT-solvers based on resolution. Since the
resolvent clauses produced by resolution are implied by the original
formula, such SAT-solvers perform semantic derivation. Suppose one
needs to solve formula $A(X,Y) \wedge B(Y,Z)$ where $X,Y,Z$ are sets
of Boolean variables. Assume also that set $Y$ is much smaller than
$X$ and $Y$. So one can view formula $A \wedge B$ as describing two
blocks ``communicating'' via variables of $Y$. Modern SAT-solvers are
based on derivation of conflict clauses. Typically, such a SAT-solver
starts deriving clauses relating internal variables of blocks $A$ and
$B$ thus losing the two-block structure of the original
formula\footnote{\input{f2ootnote}}.
------
 The satisfiability of $F_N \wedge z$
is typically checked by a resolution-based SAT-solver.
Every clause produced by resolution is implied by the original
formula. Since implication is a semantic property, this method of
solving Circuit-SAT can be viewed as semantic.
----------
We will call $T$ a trivial CTS if it consists of all $2^{|X|}$ tests.
A traditional point of view is that the only CTS for $N$ is the
trivial one. In other words, one considers testing just as sampling
the truth table of circuit $N$ that ignores its specifics.  A flaw of
this point of view does not explain why testing is so effective taking
into account that only a minuscule part of the truth table is sampled.
The existence of non-trivial CTS provides at least two reasons for
such effectiveness. First, the size of a CTS can be much smaller than
$2^{|X|}$. Second, a CTS is circuit specific. (This is due to the fact
that, as we show in Section, an SSP is formula specific. The fact that
$P$ is an SSP for formula $H$ does not mean that it is also an SSP for
a formula $Q$ logically equialent to $H$.) This means that a good set
of tests exploits the structure of circuit $N$ (which is quite obvious
for an experienced verification engineer). 
-----------
This algorithm accepts formula $F$ that is satisfiable iff $N
  \not\equiv 0$. It outputs a) formula $F^*$ logically equivalent to
  $F$ that depends only on variables of $X$ and b) a set of
  assignments to $X$ forming an SSP for $F^*$. The existence of an SSP
  for $F^*$ means that the latter is unsatisfiable and hence $N \equiv
  0$ holds.
----------
 A straightforward way to build an CTS is to generate
an SSP $P$ of $F_N \wedge z$ and then form the set of the tests
specified by points of $P$. (A point $\pnt{p} = (\pnt{x},\pnt{y},z)$
of $P$ specifies test \pnt{x}).
----------
Then
\pnt{s} can be reached from \pnt{p} by the following procedure
building a sequence of points $\ppnt{p}{1},\dots,\ppnt{p}{i}$ where
\ppnt{p}{1} = \pnt{p}. Pick the current assignment \ppnt{p}{i} (originally
$i=1$).  If \ppnt{p}{i} = \pnt{s}, then \pnt{s} is reached. Otheriwse,
an arbitrary clause $C$ of $H$ falsified by \ppnt{p}{i} is chosen. Since
\pnt{s} satisfies $C$, there is a variable $v$ such that $v \in \V{C}$
and assignments to $v$ are different in \ppnt{p}{i} and
\pnt{s}. Generate point \ppnt{p}{i+1} obtained from \ppnt{p}{i} by
flipping the value of $v$ and make \ppnt{p}{i+1} the current
assignment.
----------
 Only one assignment of \cube{x}{i} specifies the
correct execution trace for test \ppnt{x}{i} i.e. one produced by $N$
under input \ppnt{x}{i}.  All the other assignments specify erroneous
traces. 
-----------
Let $T = \s{\ppnt{x}{1},\dots,\ppnt{x}{k}}$ be a set of tests for $N$
i.e. $\ppnt{x}{i},1 \leq i \leq k$ is an assignment to $X$. Let \V{N}
denotes the variables of $N$ i.e. \V{N} = $X \cup Y \cup \s{z}$. Test
$\ppnt{x}{i}$ specifies a cube (denoted as \cube{x}{i}) that consists
of the assignments to $\mi{Vars}(N)$ sharing the same assignment
\ppnt{x}{i} to $X$.  Suppose $\cube{x}{1} \cup \dots \cube{x}{k}$
contains an SSA for formula $F_N \wedge z$. In this case $T$ is a CTS
since it proves $N \equiv 0$. The fact an SSA is a structural property
of a formula means that a non-trivial CTS is a structural property of
a circuit.
------------
To address this problem, we present
a procedure that builds a CTS for a ``projection'' of circuit $N$ onto
variables of $W$ where $X \subseteq W \subset \V{N}$. We will refer to
such a CTS as a CTSP for $N$ where 'P' stands for ``projection''. A
CTSP can be viewed as an approximation of a CTS for $N$. We will refer
to the procedure generating an CTSP as \ctsp. The main idea of \Ctsp
is to derive a simpler formula $H(W)$ from $F_N \wedge z$ and
construct an SSA of $H$ rather than $F_N \wedge z$. Formula $H$ is
derived by resolution and so it is implied by $F_N \wedge z$. The
latter fact plus the existence of SSA for $H$ entails $N \equiv
0$. (If SSA of $H$ does not exist, \Ctsp generates a counterexample
proving $N \not\equiv 0$.) A CTSP for $N$ is extracted from the SSA
built for $H$.
----------
\begin{definition}
Let $H(V)$ be a CNF formula specified by a set of clauses
\s{C_1,\dots,C_k}. $P$ = \s{\ppnt{p}{1},\dots,\ppnt{p}{m}}, $m \leq k$
is called a Stable Set of Assignments (SSA) for $H$ if for every
assignment \ppnt{p}{i} of $P$ it is true that a) \ppnt{p}{i}
falsfifies $H$ and b) there is a clause $C_j$ of $H$ falsified by
\ppnt{p}{i} such that $\nnbhd{p}{i}{C_j} \subseteq P$.
\end{definition}
----------
\begin{definition}
  Let $H(V)$ be a CNF formula specified by a set of clauses
  \s{C_1,\dots,C_k}. $P$ = \s{\ppnt{p}{1},\dots,\ppnt{p}{m}}, $m \leq
  k$ is called an SSA for $H$ with center $\sub{p}{init} \in P$ or
  just centered SSA if for every assignment \ppnt{p}{i} of $P$ it is
  true that a) \ppnt{p}{i} falsfifies $H$ and b) there is a clause
  $C_j$ of $H$ falsified by \ppnt{p}{i} such that
  $\mi{Nbhd}(\sub{p}{init},\ppnt{p}{i},C) \subseteq P$.
\end{definition}
--------
The notion of a non-trivial CTS (complete test set) is based on the
following idea. Let $T$ be a set of tests
\s{\ppnt{x}{1},\dots,\ppnt{x}{k}} where $k < 2^{|X|}$. The set of
assignments to \V{N} sharing the same assignment \ppnt{x}{i} to $X$
form a cube of $2^{|Y|+1}$ assignments. (Recall that $\V{N} = X \cup Y
\cup \s{z}$.)  Denote this set as \cube{x}{i}. Only assignment
\cube{x}{i} specifies the correct execution trace produce in $N$ under
\ppnt{x}{i}.  All other assignments can be viewed as ``erroneous''
traces. Assume that $\cube{x}{1} \cup \dots \cube{x}{k}$ contains an
SSA for formula $F_N \wedge z$. Then $T$ specifies a proof that $N
\equiv 0$ and so can be viewed as a CTS. If $T$ consists of $2^{|X|}$
tests, i.e. $T$ is a trivial CTS, then set $\cube{x}{1} \cup \dots
\cube{x}{k}$ contains the trivial SSA consisting of all assignments to
\V{F_N \wedge z}. Given an SSA of $F_N \wedge z$, one can easily
generate a CTS by extracting all different assignments to $X$ that are
present in the assignments of this SSA.
----------
\subsection{Better coverage metrics}
\sas can be used for testing complex conditionals in software.  Let us
show, for instance, how \sas can be used to address a flow of MC/DC
(Modified Condition/Decision Coverage).  MC/DC in avionics software
development guidance DO-178B and DO-178C to ensure adequate testing of
the most critical (Level A) software. Suppose that a program contains
stement ``IF ($x_1 \wedge x_2 \wedge x_3$) then .. else ...'' Here
$x_i$ is a Boolean variable specifying the value of a predicat (e.g. $
x_1 = (K < 5)$ where $K$ is an integer variable). A traditional
decision coverage just requires the presence of two test cases for
which $x_1 \wedge x_2 \wedge x_3$ evaluates to 0 and 1.  MC/DC
requires that the test suite contains tests showing that every
variable $x_i$ matters \ti{separately}. That is achieved for instance
by making the test suite constain four test cases producing
assignments 111,011,101,110 to \s{x_1,x_2,x_3}. For example,
assignments 111 and 011 show that condition $x_1$ matters. A flaw of
MC/DC is that applied to individual IF statements. So a develop can
reduce the burden of MC/DC coverage by breaking up complex
expressions. For instance, one can replace the IF statement above with
a cascade of two simpler IF staments.

The problem above can be addressed by using \sas as follows. The idea
is to require that the test suite contains test cases that form
a CTS for miters describing self-equivalence of conditionals. Consider
the IF statement above. Let $N$ be a miter describing self-equivalence
of AND gate ($x_1 \wedge x_2 \wedge x_3$) (see Figure ...). Application
of \sas to $F_N \wedge z$ where $z$ specifies the output of the miter
produce
-----------
This procedure constructs a formula $H(V)$ implied by
  $F_N \wedge z$ where $X \subseteq V \subset \V{F_N \wedge z}$ and
  tries to build an SSA for $H$. If an SSA exists, then $H$ is
  unsatisfiable and so is $F_N \wedge z$. The latter entails $N \equiv
  0$.  The SSA built by \sas specifies the set of tests $T$ consisting
  of all assignments to $X$ present in assignments of SSA. 
-------
Let $M$ be a multi-output combinational circuit. Let $N_1,\dots,N_k$
be single-output circuits obtained from $M$ that specify $k$
properties of $M$.(For instance, a circuit $N_i$ specify the property
that $M$ should not produce some outputs.)  Typically, testing is used
to verify all properties at once. That is one applies a set of tests
checking if the output produced by $M$ for a particular test displays
an incorrect behavior. For that reason, typically one uses a set of
inpus that is uniformly distributed in the space of all inputs.  An
obious flaw of this approach is that uniform distribution may not be
the most effective way to verify a \ti{particular} property.
--------
Note that the trivial SSA consisting of all assignments
is not, in general, a centered SSA.
-----
In this subsection, we consider circuits that are
non-redundant in the following sense. 
--------
\tb{\scriptsize{1}}\> $\mi{Body} = \emptyset$;  $\Fi := \emptyset$  \\
\tb{\scriptsize{2}}\> $\sub{p}{init} := \mi{PickInitAssgn}(H)$\\
\tb{\scriptsize{3}}\> $\mi{Bnd} := \s{\sub{p}{init}}$   \\
\tb{\scriptsize{4}}\>  while ($\mi{Bnd} \neq \emptyset$) \{\\
\tb{\scriptsize{5}}\Tt  $\pnt{p} := \mi{PickAssgn}(\mi{Bnd})$  \\
\tb{\scriptsize{6}}\Tt  $\mi{Bnd} := \mi{Bnd} \setminus \s{\pnt{p}}$ \\
\tb{\scriptsize{7}}\Tt  if $(\mi{SatAssgn}(\pnt{p},H))$ \\
\tb{\scriptsize{8}}\ttt   return($\pnt{p},\mi{nil},\mi{nil}$) \\
\tb{\scriptsize{9}}\Tt $C := \mi{PickFalsifClause}(H,\pnt{p})$   \\
\tb{\scriptsize{10}}\Tt $New := \nbhd{p}{C} \setminus \mi{Body}$ \\
\tb{\scriptsize{11}}\Tt $\mi{Bnd} := \mi{Bnd} \cup New$ \\
\tb{\scriptsize{12}}\Tt $\mi{Body} := \mi{Body} \cup \s{\pnt{p}}$ \\
\tb{\scriptsize{13}}\Tt $\Fi := \Fi \cup \s{(\pnt{p},C)}$ \\
\tb{\scriptsize{14}}\> return($\mi{nil},\mi{Body},\Fi$) \}\\
-----------
Given a satisfiable formula $H$, the non-deterministic procedure
\ti{BuildPath} described in Subsection~\ref{ssec:ssa_sat} (see
Figure~\ref{fig:bld_path}) builds a sequence of assignments starting
at \sub{p}{init} and ending at a satisfying assignment \pnt{s} closest
to \sub{p}{init}.  Importantly, the Hamming distance
between \ppnt{p}{i+1} and \sub{p}{init} is greater than that
between \ppnt{p}{i} and \sub{p}{init} by 1. In other words,
\ppnt{p}{i+1} is farther away from the initial assignment than \ppnt{p}{i}.
Thus, one can always reach a satisfying assignment (if any) moving
monotonically away from \sub{p}{init}.  However,
procedure \ti{BuildSSA} shown in Figure~\ref{fig:bld_ssa} does not
exploit this fact. Namely, when \ti{BuildSSA} reaches an
assignment \pnt{p} it updates set \ti{Bnd} with the assignments of
\nbhd{p}{C} (lines 10-11 of Fig.~\ref{fig:bld_ssa}). Some of the
assignments from \nbhd{p}{C} can be closer to \sub{p}{init} than
\pnt{p}. So one can optimize procedure \ti{BuildSSA} by replacing
\nbhd{p}{C} with \Nbhd{p}{p}{C}. The latter contains only the
assignments of \nbhd{p}{C} that are farther away from \sub{p}{init}
than \pnt{p}.
%
\begin{example}
  Let $V = \s{v_1,v_2,v_3,v_4}$. Let \sub{p}{init}=0000
  and \pnt{p}=0011.  Let $C =
  v_2 \vee \overline{v}_3$. Then \nbhd{p}{C}
  = \s{\ppnt{p}{1},\ppnt{p}{2}} where \ppnt{p}{1} = 0111
  and \ppnt{p}{2} = 0001. Note that assignment \ppnt{p}{2} is closer
  to \sub{p}{init} than \pnt{p}. So \Nbhd{p}{p}{C} = \s{\ppnt{p}{1}}.
\end{example}

After replacing \nbhd{p}{C} with \Nbhd{p}{p}{C}, the \ti{BuildSSA} procedure
computes a special type of SSA that we refer to as a \ti{centered} SSA.
%
\begin{definition}
  Let $H$ be a CNF formula specified by a set of clauses
  \s{C_1,\dots,C_k}. Let $P$ = \s{\ppnt{p}{1},\dots,\ppnt{p}{m}} be
  assignments to \V{H}. $P$ is called an SSA of $H$ with center
  $\sub{p}{init} \in P$ or just centered SSA if there is an AC-mapping
  \Fi such that for every assignment \ppnt{p}{i} of $P$ it is true
  that $\mi{Nbhd}(\sub{p}{init},\ppnt{p}{i},C) \subseteq P$ where $C =
  \ac{\ppnt{p}{i}}$.
\end{definition}
%
%
--------
In procedure \sas
(Section~\ref{sec:algor}), we implemented a version of SSAs called
\ti{centered} ones. As far as operation of \sas is concerned, the type
of SSA used does not matter. So, we moved the description of centered
SSPs to Section~\ref{app:cssa} of the appendix.
-------------
Consider, for instance, formula $H$ of
Example~\ref{exmp:ssa}. Let $H'$ consist of all eight 3-literal
clauses: $(\overline{x}_1 \vee \overline{x}_2 \vee
\overline{x}_3),\dots, (x_1 \vee x_2 \vee x_3)$.  Formula $H'$ has
only the trivial SSA consisting of all eight possible assignments to
\s{x_1,x_2,x_3}. This means that the SSA of Example~\ref{exmp:ssa} is
not an SSA for $H'$ even though $H' \equiv H$.
-------
\tb{\scriptsize{1}}\> $(\mi{Cnfl},\pnt{a}) = \mi{RunBcp}(G,\pnt{a},L)$ \\
\tb{\scriptsize{2}}\> if ($\mi{Cnfl}$) \{\\
\tb{\scriptsize{3}}\Tt  $C := \mi{CnflCls}(G,\pnt{a},L)$\\
\tb{\scriptsize{4}}\Tt  $ G := G \cup \s{C}$\\
\tb{\scriptsize{5}}\Tt  return($\mi{nil},\s{C},\s{\pnt{v}}$)~\}\\
$---------------$ \\
\tb{\scriptsize{6}}\> $(\pnt{v},\Fi,P) := \mi{BldSSA}(G,\pnt{a}))$\\
\tb{\scriptsize{7}}\> if ($P = \mi{nil}$)\{  \\
\tb{\scriptsize{8}}\Tt if ($|\mi{\pnt{a}}| = |W|$) \\
\tb{\scriptsize{9}}\ttt return($\pnt{a} \cup \pnt{v},\mi{nil},\mi{nil}$) \}\\
\tb{\scriptsize{10}}\> else \{\\
\tb{\scriptsize{11}}\Tt $(G,\Fi)\!:=\!\mi{Normalize}(G,\Fi,\!P,\!\pnt{a},\!L)$\\
\tb{\scriptsize{12}}\Tt return($\mi{nil},\Fi,P$) \}\\
$---------------$ \\
\tb{\scriptsize{13}}\>  $w := \mi{PickVar}(W,\pnt{a})$    \\
\tb{\scriptsize{14}}\>  $\pnt{a}_0 := \mi{AddDecLvl}(\pnt{a},\!(w=0)\!,L\!+\!1)$ \\
\tb{\scriptsize{15}}\>  ($S,\Fi_0,P_0):= \mi{SemStr}(G,\pnt{a}_0,L\!+\!1)$ \\
\tb{\scriptsize{16}}\> if ($S \neq \mi{nil}$) return($S,\mi{nil},\mi{nil}$) \\
\tb{\scriptsize{17}}\> if ($w\!\not\in \V{\Fi_0(P_0)}$) \\
\tb{\scriptsize{18}}\Tt    return($\mi{nil},\!\Fi_0,\!P_0$) \\[4pt]
\tb{\scriptsize{19}}\>  $\pnt{a}_1 := \mi{AddDecLvl}(\pnt{a},\!(w=1)\!,L\!+\!1)$ \\
\tb{\scriptsize{20}}\>  ($S,\Fi_1,P_1) := \mi{SemStr}(G,\pnt{a}_1,L+1)$ \\
\tb{\scriptsize{21}}\> if ($S \neq \mi{nil}$) return($S,\mi{nil},\mi{nil}$) \\
\tb{\scriptsize{22}}\> $H_0 := \Fi_0(P_0)$; $H_1 := \Fi_1(P_1)$; \\
\tb{\scriptsize{23}}\> $(\Fi\!,\!P)\!:=\!\mi{ExclVar}(G,H_0,\!H_1,\!\pnt{a},w)$  \\
\tb{\scriptsize{24}}\> return($\mi{nil},\Fi,P$) \}\\
------------
To increase the number of
tests one can prove $\xi^*$ $k$ times \ti{randomizing} the choice of
initial assignments when computing SSAs. The final set of tests is
formed as $T_1 \cup \dots \cup T_k$. By randomizing computation of
SSAs one essentially combines CTSs and random testing.
-------
 SSAs are computed in a small number of clusters that
reflect rich symmetries of pigeon-hole formulas
--------
 The exclusion
  of variables of $\V{N} \setminus V$ makes $T$ ``less circuit
  specific'' than a CTS extracted from an SSA of $F_N \wedge z$. 

